Local Weak Degeneracy of Planar Graphs

Thomassen showed that planar graphs are 5-list-colourable, and that planar graphs of girth at least five are 3-list-colourable. An easy degeneracy argument shows that planar graphs of girth at least four are 4-list-colourable. In 2022, Postle and Smith-Roberge proved a common strengthening of these three results: with $g(v)$ denoting the length of a shortest cycle containing a vertex $v$, they showed that if $G$ is a planar graph and $L$ a list assignment for $G$ where $|L(v)| \geq \max\{3,8-g(v)\}$ for all $v \in V(G)$, then $G$ is $L$-colourable. Moreover, they conjectured that an analogous theorem should hold for correspondence colouring. We prove this conjecture; in fact, our main theorem holds in the still more restrictive setting of weak degeneracy, and moreover acts as a joint strengthening of the fact that planar graphs are weakly 4-degenerate (originally due to Bernshteyn, Lee, and Smith-Roberge), and that planar graphs of girth at least five are weakly 2-degenerate (originally due to Han et al.).

==> figures/tikz_library.tex <==
\makeatletter
\DeclareRobustCommand{\rvdots}{%
  \vbox{
    \baselineskip4\p@\lineskiplimit\z@
    \kern-\p@
    \hbox{.}%
    \kern0.94\p@
    \hbox{.}%
    \kern0.94\p@
    \hbox{.}%
  }}
\makeatother

\tikzset{vertex/.style={shape=circle,draw=black,fill=white,inner sep=1pt, minimum size=7pt}}

\tikzset{nvertex/.style={shape=circle,draw=black,fill=gray!50,inner sep=1pt, minimum size=7pt}}

\tikzset{precoloured/.style={shape=rectangle,draw=black,fill=white,inner sep=1pt,minimum size=7pt}}

\tikzset{white/.style={shape=circle,draw=black,fill=white,inner sep=1pt, minimum size=7pt}}

\tikzset{starnode/.style={inner sep=1pt, minimum size=7pt, star,star points=4,star point ratio=0.5, draw, fill=white}}

\tikzset{invisible/.style={shape=circle,draw=black,fill=black,inner sep=0pt, minimum size=0.1pt}}

\tikzset{paren/.style={label={[left,shift={(-2pt,-4pt)}]$($},label={[right,shift={(2pt,-4pt)}]$)$}}}

\tikzset{thickedge/.style={line width=1.2pt}}

\tikzset{tinylabel/.style={font=\tiny}}

\tikzset{elabel/.style={font=\footnotesize}}

\tikzset{wavy/.style={decorate,decoration={snake,amplitude=0.25mm,segment length=1mm}}}

